PointMixer: MLP-Mixer for Point Cloud Understanding

MLP-Mixer has newly appeared as a new challenger against the realm of CNNs and transformer. Despite its simplicity compared to transformer, the concept of channel-mixing MLPs and token-mixing MLPs achieves noticeable performance in visual recognition tasks. Unlike images, point clouds are inherently sparse, unordered and irregular, which limits the direct use of MLP-Mixer for point cloud understanding. In this paper, we propose PointMixer, a universal point set operator that facilitates information sharing among unstructured 3D points. By simply replacing token-mixing MLPs with a softmax function, PointMixer can "mix" features within/between point sets. By doing so, PointMixer can be broadly used in the network as inter-set mixing, intra-set mixing, and pyramid mixing. Extensive experiments show the competitive or superior performance of PointMixer in semantic segmentation, classification, and point reconstruction against transformer-based methods.

==> figures/fig_layer/fig_layer.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=0.85\linewidth]{figures/fig_layer/fig_layer_13.pdf}
\vspace{-2mm}
\caption{\textbf{PointMixer layer.} Given a set of points~$\mathcal{P}_i$ and their corresponding features~$\mathcal{X}_i$, PointMixer produces a new query feature vector~$\mathbf{y}_i$. In contrast to MLP-Mixer~\cite{mlp-mixer}, we utilize relative position vector~$\Delta\mathbf{p}_{i,k}$ for processing unstructured 3D points.}
\label{fig:fig_layer} 
\vspace{-4mm}
\end{figure*}

==> macro.tex <==
\newcommand{\App}[1] {Appendix \ref{app:#1}}
\newcommand{\Etal}   {et al.}

\newcommand{\chunghyun}[1]{\textcolor{orange}{#1}\PackageWarning{Chunghyun:}{#1!}}
% \newcommand{\B}[1]{\textcolor{blue}{B: #1}\PackageWarning{B:}{#1!}}
\newcommand{\todo}[1]{\textcolor{red}{Todo: #1}\PackageWarning{TODO:}{#1!}}
\newcommand{\jaesik}[1]{\textcolor{cyan}{Jaesik:#1}\PackageWarning{Jaesik:}{#1!}}

% 수식
\newcommand{\mathMesh}{\mathcal{M}}
\newcommand{\mathFace}{f}


==> section-rebuttal/Q0-thanks.tex <==
We thank \rone, \rtwo, and \rthree for their precious comments and suggestions on the paper. All reviewers noted our contributions to be ``novel and superior performance'' [\rone, \rtwo, and \textbf{R3}] and ``well-explained and supported'' [\rone and \textbf{R3}]. However, there are some issues in our presentation that we will cover in this feedback.
All references are consistent with those in the manuscript. 
The scores are WA, B, WA. 


==> section-rebuttal/Q1-ch.tex <==
%%%%%%%%%%%%%%%%% Reviewer's comments %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% [R1]: "But the analysis of the differences between PointMixer and other 3D point cloud convolution methods (e.g. PointConv[1]) is missed in the paper. The relationship between the performance increases and model complexity decreases also needs to be analyzed."
% [R2]: "For experiments, in addition to the ablation study provided, the authors should also show the performance of Transformer-based and PointNet variant methods with the proposed intra-set mixing and hierarchical-set mixing operations."
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{[R1, R2] PointMixer vs. previous studies for 3D points.}
%
%
We agree with \rone and \rtwo's arguments that there are similarities between PointMixer and existing methods (\eg, PointNet\plusplus~[55], PointConv~[80], and Point Transformer~[98]) when it comes to the \textit{intra-set} mixing only.
% We agree with \rone and \rtwo's arguments that the PointMixer layer shares similarity with existing methods (\eg, PointNet\plusplus~[55], PointConv~[80], and Point Transformer~[98]) when it comes to the \textit{intra-set} mixing only.
%
%
However, in this paper, we aim (1) to improve the network expressiveness via complementary set operations (\textit{intra/inter/hier-set} mixing), 
% (2) to develop a universal set operator for all of the operations, 
(2) to develop a universal set operator, and (3) to design a symmetric network using PointMixer.

% Although none of existing methods has been designed for \textit{inter-set} mixing and (symmetric) \textit{hier-set} mixing, we explore other versions of \textit{inter-/hier-set} mixing layers using $\operatorname{max}$ and $\operatorname{vector-attention}$ instead of $\operatorname{softmax}$ (ours) as shown in Table~\ref{table:diff-bacTo addresskbone}.
% In order to underline the importance and relevance of our novel \textit{inter/hier-set} mixing (using $\operatorname{max}$ and $\operatorname{vector-attention}$ instead of $\operatorname{softmax}$), we proposed to integrate these components into other existing backbones as shown in Table~\ref{table:diff-backbone}.
As \rone and \rtwo requested an analysis on our \textit{inter/hier-set} mixing, we integrate these components into other existing backbones, and compare those variants with our PointMixer as shown in Table~\ref{table:diff-backbone}.
Note that PointNet\plusplus and Point Transformer use $\operatorname{max}$ and $\operatorname{vector-attention}$\footnote{Since $\operatorname{vector-attention}$ with an inverse mapping (L335-337) requires many $\operatorname{scatter}$ operations, it also heavily consumes GPU memory.} for \textit{intra-set} mixing, respectively.
%
%
The results show that \textit{inter/hier-set} mixing itself consistently improves the performance of PointNet\plusplus and Point Transformer regardless of the block designs. Interestingly, our mixing scheme~($\operatorname{softmax}$) seems to be more effective than the simple operator ($\operatorname{max}$) as well as the complex  layer~($\operatorname{vector-attention}$).
%
%
% Interestingly, our mixing scheme seems to be more effective in a relatively simple operator ($\operatorname{max}$ and $\operatorname{softmax}$) than $\operatorname{vector-attention}$.
%
%
% Moreover, PointMixer shows the best trade-off between the model complexity and mIoU as a universal set operator. %  for \textit{intra-/inter-/hier-set} mixing.
%
%
% Moreover, our PointMixer outperforms PointNet\plusplus with $\operatorname{max}$-based \textit{inter-/hier-set} mixing, showing that PointMixer layer is more effective than PointNet\plusplus layer as a universal set operator for \textit{intra-/inter-/hier-set} mixing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \footnote{Since $\operatorname{vector-attention}$ with an inverse mapping (L335-337) requires too many $\operatorname{scatter}$ operations and unaffordable GPU memory, we omit the \textit{inter-/hier-set} mixing layers with $\operatorname{vector-attention}$.}

==> section-rebuttal/Q2-ch.tex <==
%%%%%%%%%%%%%%%%% Reviewer's comments %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% [R1]: "My major concern about this work is does it really can be considered as an MLPMixer? The PointMixer block is like something in the middle of Attention and point cloud convolution. I can briefly describe the PointMixer as an attention module without any information (except the relative position) from the query point. Or it can be described as a convolution layer where the features of every point help to produce their weights (and the weights are more simple, one scalar for one point). The PointMixer seems like a module that is the sub-set of both attention and convolution"
% [R2]: "As shown in Table 1, the authors consider softmax and pooling as token mixing operations. So, could we also think pointnet&pointnet++ are kinds of MLP-Mixer as well?"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\textbf{[R1, R2]~PointMixer is a 3D version of MLP-Mixer.} \
% \noindent\textbf{[R1,R2]~Positioning.} \
% In this section, we will describe the common characteristics of MLP-Mixer and PointMixer. 
% In this section, we further describe our analysis of PointMixer compared to the previous works.

\noindent\textbf{[R1, R2] PointMixer as a 3D version of MLP-Mixer.}
% According to MLP-Mixer, 
In~[68],
\textit{“MLP-Mixer contains two types of layers: one with MLPs applied independently to image patches (i.e.,~“mixing” the per-location features), and one with MLPs applied across patches (i.e.,~“mixing” spatial information).”}. Similarly, Synthesizer~[65] also claims that ``\textit{we show that Random Synthesizers are a form of MLP-Mixers. Random Synthesizers apply a weight matrix on the length dimension as a form of projection across the dimension.}''. 
% \textit{“MLP-Mixer contains two types of layers: one with MLPs applied independently to image patches (i.e.,~“mixing” the per-location features), and one with MLPs applied across patches (i.e.,~“mixing” spatial information).”}. Similarly, Synthesizer~[65] also claims that ``\textit{we show that Random Synthesizers are a form of MLP-Mixers. Random Synthesizers apply a weight matrix R on the length dimension. R is a L $\times$ L matrix and can be seen as a form of projection across the length dimension.}''. 
% As pointed by
% \rtwo, PointMixer also follows a form of both MLP-Mixer and
% Synthesizer through $\operatorname{softmax}$ function that acts as a projection across the token dimensions, \ie,~token-mixing.
Based on theses concepts, PointMixer can be seen as a form of both MLP-Mixer and
Synthesizer through $\operatorname{softmax}$ that acts as a projection across the token dimensions, \ie,~token-mixing.
% Thus, PointMixer is a 3D version of MLP-Mixer\footnote{In this context, PointNet\plusplus also can be seen as one of the simplest versions of MLP-Mixer for point cloud understanding. However, as shown in Table~\ref{table:diff-backbone}, it is outperformed by PointMixer in the set mixing schemes.}. 
% As pointed by
% \rtwo, PointMixer also follows a form of both MLP-Mixer and
% Synthesizer through $\operatorname{softmax}$ function that acts as a projection across the token dimensions, \ie,~token-mixing.
% Thus, PointMixer is a 3D version of MLP-Mixer\footnote{In this context, PointNet\plusplus also can be seen as one of the simplest versions of MLP-Mixer for point cloud understanding. However, as shown in Table~\ref{table:diff-backbone}, it is outperformed by PointMixer in the set mixing schemes.}. 

% \ch{\rone and \rtwo question the relationship between PointMixer and MLP-Mixer. It's regrettable that it sounds too strong; we agree with \rone and \rtwo. What we actually meant by the \textbf{\textbf{PointMixer}} is a simple MLP architecture for 3D points with an appropriate mixing scheme. Here, we describe our analysis of PointMixer compared to the previous works.
% %
% First, the concept of \textit{token-mixing} in the MLP-Mixer is now relaxed in recently published papers: Synthesizer~\cite{synthesizer} and MetaFormer~\cite{metaformer}. Specifically, Synthesizer claims that 
% }
% ``\textit{we show that Random Synthesizers are a form of MLP-Mixers. Random Synthesizers apply a weight matrix R on the length dimension. R is a L $\times$ L matrix and can be seen as a form of projection across the length dimension.}''. 
% As pointed by
% \rtwo, PointMixer also follows a form of both MLP-Mixer and
% Synthesizer through $\operatorname{softmax}$ function that acts as a projection across the token dimensions, \ie, token-mixing\footnote{\ch{In this context, PointNet\plusplus also can be seen as one of the simplest version of MLP-Mixer for point cloud understanding. However, as shown in Table~\ref{table:diff-backbone}, it is outperformed by PointMixer in the set mixing schemes.}}.


Moreover, MLP-Mixer variants~[5,23,38,90] also focus on the improved token-mixer.
% For instance, CycleMLP~(ICLR'22)[5] samples pixels in a cyclic style to achieves linear computational complexity of token-mixing parts.
%
% For instance, CycleMLP [5] samples pixels in a cyclic style to achieves linear computational complexity of token-mixing parts.
For example, CycleMLP [5] samples pixels in a cyclic style for linear complexity in token-mixing parts.
%
% AS-MLP~(ICLR'22)[38] \textbf{also removes token-mixing MLPs} and propose Axial Shift operations for the better local token communication.
AS-MLP [38] \textbf{also removes token-mixing MLPs}, and proposes Axial Shift operations for a better local token communication.
%
From these token-mixing analyses, the direction of PointMixer is aligned with that of MLP-Mixer variants.
% With these analyses of token-mixing designs,
%
Therefore, we respectively argue that PointMixer is a 3D version of MLP-Mixer\footnote{In this context, PointNet\plusplus also can be seen as one of the simplest versions of MLP-Mixer for point cloud understanding. However, as shown in Table~\ref{table:diff-backbone}, it is outperformed by PointMixer in the set mixing schemes.}.

% Therefore, PointMixer is a 3D version of MLP-Mixer\footnote{In this context, PointNet\plusplus also can be seen as one of the simplest versions of MLP-Mixer for point cloud understanding. However, as shown in Table~\ref{table:diff-backbone}, it is outperformed by PointMixer in the set mixing schemes.}.
% Furthermore, our simple token-mixing formulation is also relevant to the MetaFormer~(CVPR'22 oral)[92], which demonstrate simple pooling operation can outperform complex token-mixers, such as attention or token-mixing MLPs.

==> section-rebuttal/Q3-softmax.tex <==

\noindent \textbf{[R2] Softmax function is not new.}
We agree the \rtwo's comments about the $\operatorname{softmax}$ function.
In our understanding, this is one way of computing a score vector as addressed by \rthree.
%
% Rather than to focusing on the operator design itself,
Nonetheless, our paper revisits the existing module to emphasize the extended use of $k$NN graph structure.
%
While previous studies focus on the directional $k$NN graph (\textit{intra-set} mixing), PointMixer newly notices the `bi'-directional characteristics of $k$NN (\textit{inter/hier-set} mixing). Furthermore, to fully utilize this newly-revisited property, the $\operatorname{softmax}$ function can be one choice instead of using complex modules.
In conclusion, our design choice (replacement token-mixing MLPs with $\operatorname{softmax}$ function) is supported by our analysis of permutation-invariant point set operators (Sec.~\textcolor{red}{3.2}) across many recent publications~[38,92,98] and our extensive experiments (Tables~\textcolor{red}{5} and Table~\textcolor{red}{F1}). 
%
% To address \rtwo's concern, we will our generic claims with specific ones, focusing on the proposed mixing schemes.
To address \rtwo's concern, we will further describe such analysis in the final manuscript.
%
% \jaesung{In conclusion, ... ?!}
% \jaesung{In conclusion, our design choice (replacement token-mixing MLPs) is strongly supported theoretically (permutation-invariancy) and experimentally (Table2 of the manuscript) across many recent publications as well as through our extensive experiments.
% Regarding the \rone and \rtwo's concerns, we will add a new section about this issue in the final manuscript.}

% \jaesung{While recent studies focus on the new ways of token-mixing schemes, Transformer, token-, 
% our simple token-mixing formulation is also relevant to the MetaFormer~(CVPR'22 oral)[92], which demonstrates simple pooling operation can outperform complex token-mixers,~\eg, attention or token-mixing MLPs. As commented by \rtwo, softmax function for 3D points is not new. Nonetheless, this paper also envisions that simple token-mixing is `also' good for processing 3D points.}
% % Furthermore, our simple token-mixing formulation is also relevant to the MetaFormer~(CVPR'22 oral)[92], 
% % \textit{``we deliberately replace the attention module with an embarrassingly simple spatial pooling operator to conduct only the most basic token mixing. Surprisingly, we observe that the derived model achieves competitive performance.''}
% % Our ablation study in Table~\textcolor{red}{5} (bottom-right) of the manuscript consistently supports this claim. 
% % In conclusion, \textbf{we have theoretical reasons (Sec.~3.2) and reasonable supports by the concurrent papers [92,38] to exclude token-mixing MLPs from PointMixer}.
% In conclusion, \textbf{our design choice (exclusion of token-mixing MLPs) is strongly supported theoretically and experimentally across many recent publications} \jaesung{as well as through our extensive experiments}.
% Regarding the \rone and \rtwo's concerns, we will add a new section about this issue in the final manuscript.




% \noindent\textbf{[R2] PointMixer vs. PointNet\plusplus.}
% We have revisited MLP-like architectures for point cloud understanding (\eg, PointNet\plusplus), and proposed a simple but effective modification with a novel ``mixing'' scheme (\textit{inter-/hier-set} mixing).
% It is noteworthy, that unlike PointNet\plusplus and Point Transformer, our architecture allows for the construction of symmetric encoder-decoder networks which proved to be particularly pertinent for point cloud segmentation.
% % It is noteworthy that the proposed mixing scheme also enables a symmetric architecture for dense prediction, which has not been studied by a large number of previous works including PointNet\plusplus and Point Transformer for a long time.
% \jaesung{Therefore, we named our method as \textbf{\textit{PointMixer}} to emphasize the contributions of the proposed mixing schemes with MLPs.}



==> section-rebuttal/Q4-noisy.tex <==
%%%%%%%%%%%%%%%%% Reviewer's comments %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% [R3]: "It would be better to add robustness analysis, e.g. robustness to noisy points and missing points"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{[R3]~Robustness experiments on noisy point clouds.} 
% As suggested by \rthree, 
We measure the accuracy drop of Point Transformer\footnote{Since there are no available pre-trained weights of Point Transformer on both S3DIS and ModelNet40, we trained the Point Transformer ourselves with the official codes provided by the Point Transformer authors.} and PointMixer when adding random Gaussian noises ($\sigma{=}0.01$) without fine-tuning.
Table~\ref{table:rebuttal-robustness} shows that PointMixer is more robust to noisy inputs than Point Transformer.
It seems that the enlarged receptive fields (Fig.~\textcolor{red}{8} of the supplementary material) through our \textit{inter/hier-set} mixing scheme also makes the network robust to the noises.
% This is due to our various aggregations of point responses through \textit{intra/inter/hier-set} with enlarged receptive fields (Fig.~\textcolor{red}{8} of the supplementary material).
% \jaesung{As shown in Table~\ref{table:rebuttal-robustness}, our method achieves higher accuracy than Point Transformer. Note that we add ??\% random noise to the given point clouds and calculate the metrics.}
% \input{tables/supp_t1_robustness}
% \noindent\textbf{[R1]~Comparison with PointConv.} \
% \jaesung{Others cannot go to universal point set operator} In our implementation, PointMixer does not use weight banks (PAConv), heuristic point density functions (PointConv), or key-query attentions (PointTransformer). Our method purely consists of MLPs and pooling layers, which is the same as the MLP-Mixer network. Moreover, this common philosophy is consistently supported by the recent studies about MLP-Mixer variants that address the improved way of token-mixing operation similar to PointMixer. (\rone)~Accordingly, PointMixer is much closer to MLP-Mixer rather than to PointConv or attention-based studies.


% We use the best implementation of Point Transformer available in the public domain, which contains the official code provided by Point Transformer authors. The reproduced OA of Point Transformer is 93.3.

% As suggested by \rthree, we evaluate the robustness of Point Transformer\footnote{Since there are no available pre-trained weights of Point Transformer on ModelNet40, we trained the Point Transformer ourselves with the official codes provided by the Point Transformer authors for the experiments.} and PointMixer to random noises on S3DIS and ModelNet40 datasets.

==> section-rebuttal/Q5-etc.tex <==

\noindent \textbf{[R1, R2, R3] Other detailed comments.} We appreciate all the detailed comments, and will do our best to reflect on them; adding analysis [\rone, \textbf{R3}], correcting abbreviations and typos [\rone, \textbf{R3}], clarifying the storyline [\textbf{R2}].


% \noindent\textbf{[R1]~Efficiency analysis.} \
% \jaesung{Please refer to the Sec.1 of the supplementary material. PointMixer demonstrate ??\% parameter efficiency with ??\% improved accuarcy comparison with PointTransformer.}

% In this point of view, we agree with \rtwo's opinion, \textit{`PointMixer is regarded as a PointNet variant'}.
% Moreover, we also admit that \textit{`PointNet and PointNet++ can be also viewed as MLP-Mixer'}. 
% This is because all these studies only adopt MLPs, not convolutions or transformers.
%
% Nonetheless, we claim that previous PointNet variants are limited versions of MLP-Mixer. 
% While MLP-Mixer can be applied to various sets of tokens for image recognition tasks, previous PointNet variants can only process intra-set mixing. 
% This difference comes from the unstructured and unordered properties of point cloud
% In contrast to image, previous papers widely use MLP to deal with unstructured points.
% Similarly, PointMixer also revisits the usage of MLPs for point cloud understanding. 
% Typically, we newly design inter-set and hierarchical-set mixing to consider various cardinality of point sets.



% In contrast to image recognition methods, MLPs are already widely used in point cloud processing.
% In other words, this is the problem of token-mixing designs (\eg, convolution, attention, MLPs or pooling), as mentioned in MetaFormer. We admit the worries from \rone and \rtwo, \textit{`PointMixer seems like a module that is the sub-set of both attention and convolution'} and \textit{`PointMixer is more like a PointNet variant'}.
% \rone and \rtwo asked us for the clear position of PointMixer. 
% \rone typically argued that PointMixer seems like a module that is the sub-set of both attention and convolution. 
% \rtwo addressed that PointMixer is more like a PointNet variant. 
% Let us provide our opinions on the reviewers' analysis. 




==> section-rebuttal/old/Q1-js.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \jaesung{
\textbf{[R1] PointMixer as a subset of attention and conv layer?} According to Synthesizer, transformer utilize key-query similarities (\ie, attention) to update values while both MLP-Mixer and Synthesizer does utilize such concept. Accordingly, PointMixer is clearly not an attention.}

\jaesung{MLP layer is inter-changeable with 1x1 conv layer so we agree with \rone's understanding, ``it can be described as a convolution layer where the features of every point help to produce their weights.'' However, compared with recent point convolution methods, we do not use heuristic point density function (PointConv) or weight banks (PAConv) as shown in Table ??. Moreover, we revisit the merits of MLPs that can process arbitrary number of tokens (3D points) while PointConv cannot. This difference treats Pointmixer as a universal set operator for \textit{intra-/inter-/hier-set} mixing.}

==> section-rebuttal/old/Q2-js.tex <==
\noindent\jaesung{\textbf{[R2] PointMixer as a 3D version of MLP-Mixer.}
According to MLP-Mixer, “MLP-Mixer contains two types of layers: one with MLPs applied independently to image patches (\ie,~“mixing” the per-location features), and one with MLPs applied across patches (\ie,~“mixing” spatial information).”. Similarly, Synthesizer also claims that ``\textit{we show that Random Synthesizers are a form of MLP-Mixers. Random Synthesizers apply a weight matrix R on the length dimension. R is a L $\times$ L matrix and can be seen as a form of projection across the length dimension.}''. Thus, PointMixer is a 3D version of MLP-Mixer.}

\noindent\jaesung{\textbf{[R1,R2]~Token-mixing MLP is not an essential choice.}
For the permutation-equivariance (Sec.~3.2), we replace token-mixing MLPs into softmax function for PointMixer layer.
Such formulation is quite close to the concurrent work, MetaFormer (CVPR 2022, oral), \textit{``simplified token mixing (such as pooling) is enough or better than attention layers or token-mixing MLPs''}.
Our ablation study in Table~5 (bottom-right) of the manuscript constantly support this claim.
Even though such design choice can make PointMixer look closer to PointNet, however, \textbf{We have analytic~/ theoretical reasons (Sec.~3.2) and reasonable supports by the concurrent paper (Sec.~1) to exclude token-mixing MLPs from PointMixer}. We will include additional paragraphs to clearly explain this issue as the previous study (Synthesizer) did. 
}





% First, \textbf{both MLP-Mixer and PointMixer newly envision the importance of MLPs in the realm of CNNs and Transformers.}
% Similar to the image recognition tasks, recent studies about point cloud analysis proposed convolution-based schemes as well as transformer-based networks. 
% In our implementation, (\rone)~PointMixer does not use weight banks (PAConv), \jaesung{heuristic} point density functions (PointConv), or key-query attentions (PointTransformer).
% First, our method purely consists of MLPs and pooling layers, which is the same as the MLP-Mixer network. 
% (\rone)~Accordingly, PointMixer is much closer to MLP-Mixer rather than to PointConv or attention-based studies \jaesung{due to its MLP-like architecture.}

% Second, \textbf{PointMixer is a MLP-Mixer variant.}
% % According to Synthesizer, this paper also does not have token-mixing MLPs, however, this paper claims that \textit{``we show that Random Synthesizers are a form of MLP-Mixers. Random Synthesizers apply a weight matrix R on the length dimension. R is a L $\times$ L matrix and can be seen as a form of projection across the length dimension.''} As pointed by \rtwo, PointMixer also follow a form of both MLP-Mixer and Synthesizer through softmax function that act as projection across the token dimensions, \ie, token-mixing. \jaesung{Based on these previous papers, PointMixer clearly belongs to a MLP-Mixer group.}

% Third, \textbf{both PointMixer and previous MLP-Mixer successors proposed the improved way of token-mixer.} 
% \jaesung{Concretly speaking, MLP-Mixer variants for image recognition proposed axis-swap~($\text{S}^{2}$), spatial permutation~(Permutable) or unique pixel sampling (cycleMLP) to address the issues in token-mixing MLPs. Since PointMixer also proposes the efficient and permutation-invariant token-mixer, both PointMixer and previous MLP-Mixer variants share common philosophy, which can be reason for our claim, PointMixer is a MLP-Mixer variant.}



% Fourth, \textbf{both PointMixer and PointNet are MLP-like architecture.}
% We admit the worrying points by \rtwo that there are some similarities between PointNet variant and PointMixer. 
% Nonetheless, through our formulation, PointMixer can be closer to the MLP-Mixer and becomes a universal point set operator. 
% Moreover, the name of the PointMixer emphasizes various `mix' operations, such as intra-, inter-, and hierarchical-set mixing, while PointNet++ does not. 
%
% \ch{Moreover, PointMixer block (Fig.~2) differs from existing methods (\textit{e.g.}, PointNet, PointTransformer) in that a novel \textit{inter-set} mixing layer is introduced within the block.}
% \ch{Experiments (scatter-max), here.}
% We hope the \rtwo satisfied with our analysis and opinion.
%
% Regarding the \rtwo worries, we will include additional paragraphs to clearly explain this issue as the previous study (Synthesizer) did. 

% Last, \textbf{Token-mixing MLP is not an essential choice.}
% For the permutation-equivariance (Sec.~3.2), we replace token-mixing MLPs into softmax function for PointMixer layer.
% Such formulation is quite close to the concurrent work, MetaFormer (CVPR 2022, oral), \textit{``simplified token mixing (such as pooling) is enough or better than attention layers or token-mixing MLPs''}.
% Our ablation study in Table~5 (bottom-right) of the manuscript constantly support this claim.
% Even though such design choice can make PointMixer look closer to PointNet, however, \textbf{we have clear theoretical reasons (Sec.~3.2) and reasonable supports by the concurrent paper (Sec.~1) to drop out token-mixing MLPs from PointMixer}.



==> section-rebuttal/overview.tex <==
 \noindent\textbf{Overview.} \
Overall, three reviewers agree with our analysis and strength of the PointMixer design.
\rone said \textit{`The proposed symmetric transition down/up mixing module is novel.'}
\rtwo denoted our strength as \textit{``the transition layer with proposed hierarchical-set mixing could give symmetric output which is more effective for semantic segmentation tasks.''}. 
Lastly, \rthree described as \textit{``The point set operator design is novel.''} 
Besides from our novelty, \rone and \rtwo raise questions about the relevance between PointMixer and previous studies, such as PointConv, and MLP-Mixer.

==> section/5-limitation.tex <==
PointMixer network shows the best performance in dense prediction tasks, but not in object classification task.
\chunghyun{Need to be updated based on the voting results.}
% \chunghyun{Although our PointMixer layer shows impressive performance on dense prediction tasks~\cite{armeni_cvpr16,point-recon}, it still performs comparable to the state-of-the-art method, Point Transformer~\cite{point-transformer}, on object shape classification~\cite{modelnet40}. The reason is that }
Since MLP-Mixer is originally designed for image classification, we do not expect MLPs are the reason. 
Since we did not provide the reasonable explanation, we will further investigate this problem for the upgraded PointMixer design.

% Instead, we expect that $k$NN-based sampling can raise problems. As addressed in~\cite{kpconv,interpconv}, $k$NN is sensitive to the density of points' distribution while voxel hashing~\cite{mink,point-recon} is not. Since absolute-scale understanding is also important aspect in point cloud processing, it will be a good direction as a research topic.

==> tables/etc/t4_abl_neighbor.tex <==
\begin{table}[!t]
\centering
% \setlength{\tabcolsep}{4pt}
\resizebox{0.47\linewidth}{!}{
\begin{tabular}{ccclcclcc}
\Xhline{4\arrayrulewidth}

\multicolumn{3}{c}{Preserve (\checkmark)} & &
\multicolumn{2}{c}{Semantic seg} & &
\multicolumn{2}{c}{Point recon} 
\\ \cline{1-3} \cline{5-6} \cline{8-9} 

\multicolumn{3}{c}{Type of mixing set} & &  
\multirow{2}{*}{mIoU} & \multirow{2}{*}{mAcc} & &
\multirow{2}{*}{Chamf.($\downarrow$)} & \multirow{2}{*}{F1($\uparrow$)} 
\\

~~Intra~~ & ~~Inter~~ & ~~Hier~~ & &
& & &
& 
\\ \Xhline{2\arrayrulewidth}


\checkmark & & & &
0.6918 & 0.7582 & &
1.125 & 53.48 
\\ 

\checkmark & \checkmark & & &
0.6910 & 0.7565 & &
1.120& 53.50
\\ 

\checkmark & & \checkmark & &
\second{0.6926} & \second{0.7655} & &
\second{1.111} & \second{53.52} 
\\ \Xhline{2\arrayrulewidth}

\checkmark & \checkmark & \checkmark & &
\first{0.7136} & \first{0.7740} & &
\first{1.109} & \first{53.65}
\\ \Xhline{4\arrayrulewidth}



\end{tabular}}
%
% \quad %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \setlength{\tabcolsep}{4pt}
\resizebox{0.441\linewidth}{!}{
\begin{tabular}{cclcclcc}
\Xhline{4\arrayrulewidth}



\multicolumn{2}{c}{Preserve (\checkmark)} & &
\multicolumn{2}{c}{Efficiency} & &
\multicolumn{2}{c}{Accuracy} 
\\ \cline{1-2} \cline{4-5} \cline{7-8}


% TokenMLP & Softmax & &
% (M)($\downarrow$) & Hour(H) & & 
% mIoU & 
% Chamf.
% \\ \Xhline{2\arrayrulewidth}
~~Token~~ & ~~Softmax~~ & &
Param & Train & &
SemSeg & 
Recon
\\ 
MLPs & func & &
(M)($\downarrow$) & Hour(H) & & 
mIoU & 
Chamf.
\\ \Xhline{2\arrayrulewidth}


& & &
\first{6.1} & \first{40} & & 
0.5831 & 1.233
\\ 


& \checkmark & &
\first{6.1} & \second{44} & & 
\first{0.7136} & \first{1.109}
\\ \hline


\checkmark & & &
7.4 & 88 & & 
0.7105 & 1.119
\\ 


\checkmark & \checkmark & &
7.4 & 95 & & 
\second{0.7112} & \second{1.113}
\\ \Xhline{4\arrayrulewidth}

\end{tabular}}
% \vspace{-2mm}
\caption{Ablation study about types of mixing (left) and token-mixing MLPs (right).}
\label{table:ablation-operator}
\vspace{-4mm}
\end{table}

==> tables/etc/t6_abl_tokenmix.tex <==
% \begin{table}[!t]
% \setlength{\tabcolsep}{4pt}
% \resizebox{0.50\linewidth}{!}{
% \begin{tabular}{ccclcclcc}
% \Xhline{4\arrayrulewidth}

% \multicolumn{3}{c}{Preserve (\checkmark)} & &
% \multicolumn{2}{c}{Semantic seg} & &
% \multicolumn{2}{c}{Point recon} 
% \\ \cline{1-3} \cline{5-6} \cline{8-9} 

% \multicolumn{3}{c}{Mix of what?} & &  
% \multirow{2}{*}{mIoU} & \multirow{2}{*}{mAcc} & &
% \multirow{2}{*}{Chamf.($\downarrow$)} & \multirow{2}{*}{F1($\uparrow$)} 
% \\

% Channel & Token & Softmax & &
% & & &
% & 
% \\ \Xhline{2\arrayrulewidth}


% \checkmark & & & &
% 0.5831 & 0.6647 & &
% 1.233 & 48.55 
% \\ 

% \checkmark & \checkmark & & &
% \second{0.7105} & \second{0.7733} & & 
% \second{1.119} & \second{53.27} 
% \\ \Xhline{2\arrayrulewidth}

% \checkmark & & \checkmark & &
% \first{0.7136} & \first{0.7740} & &
% \first{1.109} & \first{53.65}
% \\ \Xhline{4\arrayrulewidth}

% \end{tabular}
% }
% % \vspace{-2mm}
% \caption{\textbf{Ablation study about token-mixing MLPs.}}
% \label{table:ablation-token-mix}
% \end{table}

%%%%%%%

\begin{table}[!t]
\setlength{\tabcolsep}{4pt}
\resizebox{0.40\linewidth}{!}{
\begin{tabular}{cclcclcc}
\Xhline{4\arrayrulewidth}



\multicolumn{2}{c}{Preserve (\checkmark)} & &
Param & Train & &
SemSeg & 
Recon
\\ \cline{1-2} \cline{4-5} \cline{7-8}


TokenMLP & Softmax & &
(M)($\downarrow$) & Hour(H) & & 
mIoU & 
Chamf.
\\ \Xhline{2\arrayrulewidth}


& & &
\first{6.1} & \first{40} & & 
0.5831 & 1.233
\\ 


& \checkmark & &
\first{6.1} & \second{44} & & 
\first{0.7136} & \first{1.109}
\\ \hline


\checkmark & & &
7.4 & 88 & & 
0.7105 & 1.119
\\ 


\checkmark & \checkmark & &
7.4 & 95 & & 
\second{0.7112} & \second{1.113}
\\ \Xhline{4\arrayrulewidth}

\end{tabular}}
% \vspace{-2mm}
\caption{\textbf{Ablation study about token-mixing MLPs.}}
\label{table:ablation-token-mix}
\end{table}

==> tables/supp_t0_diff_backbone.tex <==
\begin{table}[!t]
\caption{Semantic segmentation results of existing methods with the proposed inter-/hier-set mixing schemes on the S3DIS dataset. Note that `$\operatorname{max}$' represents PointNet\plusplus block using maxpool, `$\operatorname{attn}$' means the vector-attention based Point Transformer block, and `$\operatorname{softmax}$' implies our PointMixer block.}
\vspace{-3.5mm}
\label{table:diff-backbone}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccll}
\toprule
Method & Intra & Inter/Hier & Param. (M) & mIoU $(\%)$ \\
\midrule
\rowcolor{gray!20} PointNet\plusplus & $\operatorname{max}$ & \redxmark & ~~2.0 & 57.3 \\
& $\operatorname{max}$ & $\operatorname{max}$ & ~~2.3 (\textcolor{purple}{$\uparrow$ 0.3}) & 62.7 (\textcolor{teal}{$\uparrow$ 5.4}) \\ % hwang 
& $\operatorname{max}$ & $\operatorname{attn}$ & ~~8.3 (\textcolor{purple}{$\uparrow$ 6.3}) & 57.8 (\textcolor{teal}{$\uparrow$ 0.5}) \\
& $\operatorname{max}$ & $\operatorname{softmax}$ & ~~2.7 (\textcolor{purple}{$\uparrow$ 0.7}) & 66.9 (\textcolor{teal}{$\uparrow$ 9.6}) \\

\midrule

\rowcolor{gray!20} PointTransformer$^{\textcolor{red}{3}}$ & $\operatorname{attn}$ & \redxmark & ~~7.8 & 70.0 \\

& $\operatorname{attn}$ & $\operatorname{max}$ & ~~8.1 (\textcolor{purple}{$\uparrow$ 0.3}) & 70.2 (\textcolor{teal}{$\uparrow$ 0.2}) \\

& $\operatorname{attn}$ & $\operatorname{attn}$ & 14.1 (\textcolor{purple}{$\uparrow$ 6.3}) & 70.1 (\textcolor{teal}{$\uparrow$ 0.1}) \\

& $\operatorname{attn}$ & $\operatorname{softmax}$ & ~~8.5 (\textcolor{purple}{$\uparrow$ 0.7}) & 70.3 (\textcolor{teal}{$\uparrow$ 0.3}) \\

\midrule

\rowcolor{yellow!20} PointMixer (ours) & $\operatorname{softmax}$ & $\operatorname{softmax}$ & ~~6.1 & 71.4 \\

\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table}


% \begin{table}[!t]
% \caption{Semantic segmentation results of existing methods with the proposed inter-/hier-set mixing schemes on the S3DIS dataset. Note that `$\operatorname{max}$' represents PointNet\plusplus block using maxpool, `$\operatorname{attn}$' means the vector-attention based PointTransformer block, and `$\operatorname{softmax}$' implies our PointMixer block.}
% \vspace{-3.5mm}
% \label{table:diff-backbone}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccrcc}
% \toprule
% Method & Intra & Inter/Hier & Param. & mAcc $(\%)$ & mIoU $(\%)$ \\
% \midrule
% \rowcolor{gray!20} PointNet\plusplus & $\operatorname{max}$ & \redxmark & 2.0M & 63.5 & 57.3 \\
% & $\operatorname{max}$ & $\operatorname{max}$ & 2.3M & 70.6 (\textcolor{teal}{$\uparrow$ 7.1}) & 62.7 (\textcolor{teal}{$\uparrow$ 4.4}) \\ % hwang 
% & $\operatorname{max}$ & $\operatorname{attn}$ & 8.3M & 66.1 (\textcolor{teal}{$\uparrow$ 2.6}) & 57.8 (\textcolor{teal}{$\uparrow$ 0.5}) \\
% & $\operatorname{max}$ & $\operatorname{softmax}$ & 2.7M & 74.3 (\textcolor{teal}{$\uparrow$ 10.8}) & 66.9 (\textcolor{teal}{$\uparrow$ 9.6}) \\
% \midrule
% \rowcolor{gray!20} PointTrans.$^{\textcolor{red}{3}}$ & $\operatorname{attn}$ & \redxmark & 7.8M & 76.5 & 70.4 \\
% & $\operatorname{attn}$ & $\operatorname{max}$ & 8.1M & 76.2 & 70.2 (\textcolor{purple}{$\downarrow$ 0.2}) \\
% & $\operatorname{attn}$ & $\operatorname{attn}$ & 14.1M &  & ch \\
% & $\operatorname{attn}$ & $\operatorname{softmax}$ & 8.5M & 76.8 & 70.3 (\textcolor{purple}{$\downarrow$ 0.1}) \\
% \midrule
% \rowcolor{yellow!20} PointMixer & $\operatorname{softmax}$ & $\operatorname{softmax}$ & 6.1M  & 77.4 & 71.4 \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-3mm}
% \end{table}

==> tables/supp_t1_robustness.tex <==
\begin{table}[!t]
\caption{Robustness experiments with random noises. 
% `PT' and `PM' denote Point Transformer and PointMixer, respectively.
}
\vspace{-3.5mm}
\label{table:rebuttal-robustness}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|cc}
\toprule
& Add noise & \multicolumn{1}{c|}{Semseg (S3DIS)} & \multicolumn{2}{c}{Classification (ModelNet40)} \\ 
& ($\sigma{=}0.01$) & mIoU $(\%)$ & mAcc $(\%)$ & OA $(\%)$ \\
\midrule

\rowcolor{gray!20} PointTransformer$^{\textcolor{red}{3}}$ & & 70.0~~~~~~~~~~~~~~ & 91.1~~~~~~~~~~~~ & 93.3~~~~~~~~~~~~ \\

& \checkmark & 55.5 (\textcolor{purple}{$\downarrow$ 14.5}) & 89.9 (\textcolor{purple}{$\downarrow$ 1.2}) & 92.4 (\textcolor{purple}{$\downarrow$ 0.9}) \\

\midrule

\rowcolor{yellow!20} PointMixer (ours) & & 71.4~~~~~~~~~~~~~~ & 91.4~~~~~~~~~~~~~& 93.6~~~~~~~~~~~~~\\

& \checkmark & 58.7 (\textcolor{purple}{$\downarrow$ 12.7}) & 91.0 (\textcolor{purple}{$\downarrow$ 0.4}) & 92.7 (\textcolor{purple}{$\downarrow$ 0.9}) \\

% \multirow{3}{*}[-0.5ex]{PointTransformer} & \redxmark & - & 70.4 \\
% & \greencheck~(max) &  & (running) \\
% & \greencheck~(softmax) &  & (running) \\
% \midrule
% PointMixer (ours) & \greencheck~(softmax) & - & 71.4 \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table}


% \begin{table}[!t]
% \caption{Robustness experiments with random noise injection.}
% \vspace{-3.5mm}
% \label{table:rebuttal-robustness}
% \centering
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|cc|cc}
%     \toprule
%     \multirow{2}{*}[-0.5ex]{Method} & \multicolumn{2}{c|}{S3DIS} & \multicolumn{2}{c}{ModelNet40} \\ 
%     & mAcc $(\%)$ & mIoU $(\%)$ & mAcc $(\%)$ & OA $(\%)$ \\
%     \midrule
%     PointTrans. & 76.5~$\rightarrow$~**.* & 70.4~$\rightarrow$~**.* & 91.1~$\rightarrow$~89.9 & 93.3~$\rightarrow$~92.4 \\
%     \rowcolor{yellow!20} PointMixer & 77.4~$\rightarrow$~**.* & 71.4~$\rightarrow$~**.* & 91.4~$\rightarrow$~91.0 & 93.6~$\rightarrow$~92.7 \\
%     % \multirow{3}{*}[-0.5ex]{PointTransformer} & \redxmark & - & 70.4 \\
%     % & \greencheck~(max) &  & (running) \\
%     % & \greencheck~(softmax) &  & (running) \\
%     % \midrule
%     % PointMixer (ours) & \greencheck~(softmax) & - & 71.4 \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-4mm}
% \end{table}

% \begin{table}[!t]
% \caption{Robustness experiments with random noise injection.}
% \vspace{-3.5mm}
% \label{table:rebuttal-robustness}
% \centering
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|cccc}
%     \toprule
%     \multirow{2}{*}[-0.5ex]{Method} & \multicolumn{2}{c}{mIoU (\%)} & \multicolumn{2}{c}{OA (\%)} \\
%     \cmidrule{2-5}
%     & w/o noise & w/ noise & w/o noise & w/ noise \\
%     \midrule
%     PointTrans.~~~~& 70.4 & **.* (\textcolor{purple}{$\downarrow$ **.*}) & 93.3 & 92.4 (\textcolor{purple}{$\downarrow$ 0.9})\\
%     \rowcolor{yellow!20} PointMixer & 71.4 & **.* (\textcolor{purple}{$\downarrow$ **.*}) & 93.6 & **.* (\textcolor{purple}{$\downarrow$ **.*})\\
%     % \multirow{3}{*}[-0.5ex]{PointTransformer} & \redxmark & - & 70.4 \\
%     % & \greencheck~(max) &  & (running) \\
%     % & \greencheck~(softmax) &  & (running) \\
%     % \midrule
%     % PointMixer (ours) & \greencheck~(softmax) & - & 71.4 \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-4mm}
% \end{table}



% \begin{table}[!t]
% \caption{Robustness experiments with random noise injection.}
% \vspace{-3.5mm}
% \label{table:rebuttal-robustness}
% \centering
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|cc|cc|cc}
%     \toprule
%     Method & \multicolumn{2}{c|}{mIoU (\%)} & \multicolumn{2}{c|}{OA (\%)} & \multicolumn{2}{c}{mAcc (\%)} \\
%     \midrule
%     PointTrans. & 70.4 & **.* (\textcolor{purple}{$\downarrow$ **.*}) & 93.3 & 92.4 (\textcolor{purple}{$\downarrow$ 0.9}) & 91.1 & 89.9 (\textcolor{purple}{$\downarrow$ 1.2})\\
%     \rowcolor{yellow!20} PointMixer & 71.4 & **.* (\textcolor{purple}{$\downarrow$ **.*}) & 93.6 & **.* (\textcolor{purple}{$\downarrow$ **.*}) & 91.4 & \\
%     % \multirow{3}{*}[-0.5ex]{PointTransformer} & \redxmark & - & 70.4 \\
%     % & \greencheck~(max) &  & (running) \\
%     % & \greencheck~(softmax) &  & (running) \\
%     % \midrule
%     % PointMixer (ours) & \greencheck~(softmax) & - & 71.4 \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-4mm}
% \end{table}

% \begin{table}[!t]
% \caption{Robustness experiments with random noise injection.}
% \vspace{-3.5mm}
% \label{table:rebuttal-robustness}
% \centering
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|c|c|c}
%     \toprule
%     Method & mIoU $(\%)$ & OA $(\%)$ & mAcc $(\%)$ \\
%     \midrule
%     PointTrans.~ & 70.4~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 93.3~$\rightarrow$~92.4 (\textcolor{purple}{$\downarrow$ 0.9}) & 91.1~$\rightarrow$~89.9 (\textcolor{purple}{$\downarrow$ 1.2})\\
%     \rowcolor{yellow!20} PointMixer & 71.4~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 93.6~$\rightarrow$~92.7 (\textcolor{purple}{$\downarrow$ 0.9}) & 91.4~$\rightarrow$~91.0 (\textcolor{purple}{$\downarrow$ 0.4}) \\
%     % \multirow{3}{*}[-0.5ex]{PointTransformer} & \redxmark & - & 70.4 \\
%     % & \greencheck~(max) &  & (running) \\
%     % & \greencheck~(softmax) &  & (running) \\
%     % \midrule
%     % PointMixer (ours) & \greencheck~(softmax) & - & 71.4 \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-4mm}
% \end{table}

% \begin{table}[!t]
% \caption{Robustness experiments with random noises. `PT' and `PM' denote Point Transformer and PointMixer, respectively.}
% \vspace{-3.5mm}
% \label{table:rebuttal-robustness}
% \centering
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|cc|cc}
%     \toprule
%     & \multicolumn{2}{c|}{Segmentation (S3DIS)} & \multicolumn{2}{c}{Classification (ModelNet40)} \\ 
%     & mAcc $(\%)$ & mIoU $(\%)$ & mAcc $(\%)$ & OA $(\%)$ \\
%     \midrule
%     PT$^{\textcolor{red}{3}}$ & 76.5~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 70.4~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 91.1~$\rightarrow$~89.9 (\textcolor{purple}{$\downarrow$ 1.2}) & 93.3~$\rightarrow$~92.4 (\textcolor{purple}{$\downarrow$ 0.9}) \\
%     \rowcolor{yellow!20} PM & 77.4~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 71.4~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 91.4~$\rightarrow$~91.0 (\textcolor{purple}{$\downarrow$ 0.4}) & 93.6~$\rightarrow$~92.7 (\textcolor{purple}{$\downarrow$ 0.9}) \\
%     % \multirow{3}{*}[-0.5ex]{PointTransformer} & \redxmark & - & 70.4 \\
%     % & \greencheck~(max) &  & (running) \\
%     % & \greencheck~(softmax) &  & (running) \\
%     % \midrule
%     % PointMixer (ours) & \greencheck~(softmax) & - & 71.4 \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-4mm}
% \end{table}

% \begin{table}[!t]
% \caption{Robustness experiments with random noise injection.}
% \vspace{-3.5mm}
% \label{table:rebuttal-robustness}
% \centering
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|cc|cc}
%     \toprule
%     \multirow{2}{*}[-0.5ex]{Method} & \multicolumn{2}{c|}{S3DIS} & \multicolumn{2}{c}{ModelNet40} \\ 
%     & mAcc $(\%)$ & mIoU $(\%)$ & mAcc $(\%)$ & OA $(\%)$ \\
%     \midrule
%     PointTrans. & 76.5~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 70.4~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 91.1~$\rightarrow$~89.9 (\textcolor{purple}{$\downarrow$ 1.2}) & 93.3~$\rightarrow$~92.4 (\textcolor{purple}{$\downarrow$ 0.9}) \\
%     \rowcolor{yellow!20} PointMixer & 77.4~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 71.4~$\rightarrow$~**.* (\textcolor{purple}{$\downarrow$ *.*}) & 91.4~$\rightarrow$~91.0 (\textcolor{purple}{$\downarrow$ 0.4}) & 93.6~$\rightarrow$~92.7 (\textcolor{purple}{$\downarrow$ 0.9}) \\
%     % \multirow{3}{*}[-0.5ex]{PointTransformer} & \redxmark & - & 70.4 \\
%     % & \greencheck~(max) &  & (running) \\
%     % & \greencheck~(softmax) &  & (running) \\
%     % \midrule
%     % PointMixer (ours) & \greencheck~(softmax) & - & 71.4 \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-4mm}
% \end{table}

==> tables/supp_t2_comparison.tex <==
% \begin{wraptable}{r}{0.60\textwidth}
\begin{table}[!t]
\centering
\caption{Technical comparisons.}
\vspace{-3mm}
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{lcccccc}

\Xhline{4\arrayrulewidth} 

\multirow{2}{*}[-0.5ex]{Method} & \multirow{2}{*}[-0.5ex]{~~~Locality~~~} & \multicolumn{3}{c}{~Set operator~} & ~~~Symmetric~~~ & \multirow{2}{*}[-0.5ex]{~Token-mix~} 
\\ \cline{3-5}

 &  & Intra & ~Inter~ & Hier & pyramid arch & 
\\ \Xhline{2\arrayrulewidth} 
 

PointNet\plusplus & \greencheck & \greencheck & \redxmark & \redxmark & \redxmark & Pooling 
\\ 

PointConv & \greencheck & \greencheck & \redxmark & \redxmark & \redxmark & Conv
\\ 

PointTrans & \greencheck & \greencheck & \redxmark & \redxmark & \redxmark & Self-attn 
\\ 

\rowcolor{yellow!20} PointMixer & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & Softmax 
\\ \Xhline{4\arrayrulewidth} 

\end{tabular}
}
% \label{table:compare}
\end{table}
